Data-Driven Smart Maintenance of Historic Buildings

Digital transformation in the built environment offers new opportunities to improve building maintenance through data-driven approaches. Smart monitoring, predictive modeling, and artificial intelligence can enhance decision-making and enable proactive strategies. The preservation of historic buildings is an important scenario where preventive maintenance is essential to ensure long-term sustainability while protecting heritage values. This thesis presents a comprehensive solution for data-driven smart maintenance of historic buildings, integrating Internet of Things (IoT), cloud computing, edge computing, ontology-based data modeling, and machine learning to improve indoor climate management, energy efficiency, and conservation practices. This thesis advances data-driven conservation of historic buildings by combining smart monitoring, digital twins, and artificial intelligence. The proposed methods enable preventive maintenance and pave the way for the next generation of heritage conservation strategies.

==> abstract.tex <==
%%% Abstract.tex --- 
%% 
%% Filename: Abstract.tex
%% Description: 
%% Author: Ola Leifler
%% Maintainer: 
%% Created: Thu Oct 14 13:34:11 2010 (CEST)
%% Version: $Id$
%% Version: 
%% Last-Updated: Fri Jan 14 08:48:50 2022 (+0100)
%%           By: Ola
%%     Update #: 6
%% URL: 
%% Keywords: 
%% Compatibility: 
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Commentary: 
%% 
%% 
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Change log:
%% 
%% 
%% RCS $Log$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Code:

% ✅✅
Digital transformation in the built environment offers new opportunities to improve building maintenance through data-driven approaches. Smart monitoring, predictive modeling, and artificial intelligence can enhance decision-making and enable proactive strategies. The preservation of historic buildings is an important scenario where preventive maintenance is essential to ensure long-term sustainability while protecting heritage values. This thesis presents a comprehensive solution for data-driven smart maintenance of historic buildings, integrating Internet of Things (IoT), cloud computing, edge computing, ontology-based data modeling, and machine learning to improve indoor climate management, energy efficiency, and conservation practices.

To enable long-term environmental monitoring, a scalable digitalization solution is developed in Paper I, integrating an IoT-based sensing system with edge and cloud computing. Field deployments confirm the long-run reliability of the system in supporting real-time and historical data analysis for maintenance decisions. Papers II and III further introduce the concept of parametric digital twins, incorporating ontology-based data models to ensure a consistent representation of building structures, systems, and environmental conditions. Case studies at the City Theatre of Norrköping and Löfstad Castle in Östergötland, Sweden, validate the effectiveness of digital twins in identifying indoor climate risks and guiding conservation strategies.

Based on the collected data, Papers IV and VI explore deep learning methods for building energy forecasting. Paper IV evaluates state-of-the-art deep learning architectures for point and probabilistic multi-horizon forecasting, showing that incorporating future exogenous factors improves prediction accuracy. It also highlights how different building operating modes impact forecasting performance. Paper VI integrates deep learning with digital twins to identify energy-saving opportunities and optimize operations.

Papers V and VII focus on predictive modeling for indoor climate management. Paper VII proposes an edge-centric approach as an alternative to cloud-centric solutions, ensuring low latency and data privacy. Paper V explores federated deep learning as a privacy-aware solution for decentralized indoor climate forecasting. A comparative study of federated learning algorithms demonstrates that federated models can achieve prediction accuracy comparable to centralized learning while preserving data privacy. These findings offer practical insights for managing heterogeneous, distributed environmental data to support sustainable building operations.

This thesis advances data-driven conservation of historic buildings by combining smart monitoring, digital twins, and artificial intelligence. The proposed methods enable preventive maintenance and pave the way for the next generation of heritage conservation strategies.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Abstract.tex ends here


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "demothesis"
%%% End: 


==> acknowledgments.tex <==
%%% Acknowledgments.tex<2> --- 
%% 
%% Filename: Acknowledgments.tex<2>
%% Description: 
%% Author: Ola Leifler
%% Maintainer: 
%% Created: Wed Nov 10 09:45:11 2010 (CET)
%% Version: $Id$
%% Version: 
%% Last-Updated: Tue Jun 21 13:28:03 2016 (+0200)
%%           By: Ola Leifler
%%     Update #: 6
%% URL: 
%% Keywords: 
%% Compatibility: 
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Commentary: 
%% 
%% 
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Change log:
%% 
%% 
%% RCS $Log$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Code:

\swedishenglish{\chapter*{Författarens tack}}{\chapter*{Acknowledgments}}
% ✅✅

First, I would like to express my sincere gratitude to my supervisors, Professor Shaofang Gong and Senior Associate Professor Magnus Karlsson. Shaofang gave me the opportunity to pursue this research and has provided invaluable guidance, expertise, support, and patience throughout my journey. Magnus consistently offered insightful feedback and constructive criticism that encouraged me to strive for excellence.

I am also thankful to Dr.~Yu Liu for his thoughtful advice and encouragement. I extend my appreciation to Gustav Knutsson and other colleagues at the Division of Physics, Electronics, and Mathematics, as well as the Department of Science and Technology. Their stimulating discussions, collaborative spirit, and generosity in sharing knowledge have greatly enriched this experience.

Special thanks go to our research collaborators from Uppsala University Campus Gotland, RISE in Linköping, Norrevo Fastigheter AB in Norrköping, and Östergötlands museum in Linköping. Their expertise, cooperation, and openness in sharing resources and insights have been essential to the success of this research.

Finally, I am deeply grateful to my parents and parents-in-law for their unwavering love and support. To my wife, Dr.~Chi Zhang, thank you for your patience, understanding, and wisdom, which continue to inspire me. My son, Leo, deserves special mention for bringing joy, laughter, and boundless energy into my life.

This research was financially supported by the Swedish Energy Agency (Energimyndigheten) and the Swedish Innovation Agency (Vinnova).

\vspace{5mm}

\noindent{Zhongjun Ni}

\noindent{Västerås, March 2025}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Acknowledgments.tex<2> ends here

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "demothesis"
%%% End: 


==> listofabbreviations.tex <==
\chapter*{Acronyms and Abbreviations}

\begingroup

\renewcommand{\arraystretch}{1.3}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[!ht]
\begin{tabular}{@{}llll@{}}
1F         &  &  & first floor                                                        \\
2F         &  &  & second floor                                                       \\
3D         &  &  & three dimensional                                                  \\
AI         &  &  & artificial intelligence                                            \\
ANN        &  &  & artificial neural network                                          \\
API        &  &  & application programming interface                                  \\
BF         &  &  & basement                                                           \\
CET        &  &  & Central European Time                                              \\
Ch.        &  &  & channel                                                            \\
CM         &  &  & compute module                                                     \\
CMA        &  &  & central moving average                                             \\
CNN        &  &  & convolutional neural network                                       \\
CO\textsubscript{2}        &  &  & carbon dioxide                                     \\
CSV        &  &  & comma-separated values                                             \\
CV-RMSE    &  &  & coefficient of variation of the root mean square error             \\
DTDL       &  &  & digital twins definition language                                  \\
EDA        &  &  & exploratory data analysis                                          \\
El.        &  &  & electricity                                                        \\
FEDformer  &  &  & frequency   enhanced decomposed transformer                        \\
FedAdagrad &  &  & federated adaptive optimization using Adagrad                      \\
FedAdam    &  &  & federated adaptive optimization using Adam                         \\
FedAvg     &  &  & federated averaging                                                \\
FedAvgM    &  &  & federated averaging with server momentum                           \\
FedMedian  &  &  & federated median                                                   \\
FedYogi    &  &  & federated adaptive optimization using Yogi                         \\
FL         &  &  & federated learning                                                
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[!ht]
\begin{tabular}{@{}llll@{}}
GF      &  &  & ground floor                                                  \\
GRU     &  &  & gated recurrent unit                                          \\
GWL     &  &  & groundwater level                                             \\
HVAC    &  &  & heating, ventilation, and air-conditioning                    \\
IID     &  &  & independent and identically distributed                       \\
IoT     &  &  & Internet of Things                                            \\
LR      &  &  & linear regression                                             \\
LSTM    &  &  & long short-term memory                                        \\
LTE     &  &  & long-term evolution                                           \\
MLP     &  &  & multilayer perceptron                                         \\
MR      &  &  & mixing ratio                                                  \\
N-BEATS &  &  & neural basis expansion analysis time series                   \\
N-HiTS  &  &  & neural hierarchical interpolation for time series             \\
NMBE    &  &  & normalized mean bias error                                    \\
pcs     &  &  & pieces                                                        \\
PM      &  &  & particulate matter                                            \\
ppm     &  &  & parts per million                                             \\
RDF     &  &  & resource description framework                                \\
RH      &  &  & relative humidity                                             \\
RNN     &  &  & recurrent neural network                                      \\
SLA     &  &  & service level agreement                                       \\
SMHI    &  &  & Swedish Meteorological and Hydrological Institute             \\
SN      &  &  & seasonal naïve                                                \\
SoC     &  &  & system-on-chip                                                \\
SPARQL  &  &  & {\color[HTML]{474747} SPARQL protocol and RDF query language} \\
SQL     &  &  & structured query language                                     \\
TCN     &  &  & temporal convolutional network                                \\
TF      &  &  & transformer                                                   \\
TFT     &  &  & temporal fusion transformer                                   \\
TiDE    &  &  & time-series  dense encoder                                    \\
TSMixer &  &  & time-series mixer                                             \\
UUID    &  &  & universally unique identifier                                
\end{tabular}
\end{table}

% \begin{table}[!h]
% \begin{tabular}{@{}llll@{}}
% 3D      &  &  & three dimensional                                      \\
% AI      &  &  & artificial intelligence                                \\
% ANOVA   &  &  & one-way analysis of variance                           \\
% API     &  &  & application programming interface                      \\
% BIM     &  &  & building information modeling                          \\
% BMS     &  &  & building management system                             \\
% CO\textsubscript{2}     &  &  & carbon dioxide                                         \\
% CV-RMSE &  &  & coefficient of variation of the root mean square error \\
% EDA     &  &  & exploratory data analysis                              \\
% GRU     &  &  & gated recurrent unit                                   \\
% HVAC    &  &  & heating, ventilation, and air conditioning             \\
% ID      &  &  & identity                                               \\
% IoT     &  &  & Internet of Things                                     \\
% LR      &  &  & linear regression                                      \\
% LSTM    &  &  & long short-term memory                                 \\
% N-HiTS  &  &  & hierarchical interpolation for time series forecasting \\
% NMBE    &  &  & normalized mean bias error                             \\
% RH      &  &  & relative humidity                                      \\
% SMHI    &  &  & Swedish Meteorological and Hydrological Institute      \\
% TCN     &  &  & temporal   convolutional network                       \\
% TF      &  &  & transformer                                            \\
% TFT     &  &  & temporal fusion transformer                           
% \end{tabular}
% \end{table}

\endgroup

==> listofpublications.tex <==
\chapter*{List of Publications}

\textbf{Papers included in this thesis:}

\vspace{3mm}

\noindent{Peer reviewed journal papers}
{%\footnotesize
\begin{enumerate}[{[I]}]
  \item \textbf{Z. Ni}, Y. Liu, M. Karlsson, and S. Gong, “A Sensing System Based on Public Cloud to Monitor Indoor Environment of Historic Buildings,” \textit{Sensors}, vol. 21, no. 16, 2021.
  \item \textbf{Z. Ni}, Y. Liu, M. Karlsson, and S. Gong, “Enabling Preventive Conservation of Historic Buildings Through Cloud-based Digital Twins: A Case Study in the City Theatre, Norrköping,” \textit{IEEE Access}, vol. 10, pp. 90924--90939, 2022.
  \item \textbf{Z. Ni}, J. Hupkes, P. Eriksson, G. Leijonhufvud, M. Karlsson, and S. Gong, “Parametric Digital Twins for Preserving Historic Buildings: A Case Study at Löfstad Castle in Östergötland, Sweden,” \textit{IEEE Access}, vol. 13, pp. 3371--3389, 2025.
  \item \textbf{Z. Ni}, C. Zhang, M. Karlsson, and S. Gong, “A study of deep learning-based multi-horizon building energy forecasting,” \textit{Energy and Buildings}, vol. 303, 2024.
  \item \textbf{Z. Ni}, M. Karlsson, and S. Gong, “A study of federated deep learning for building indoor climate forecasting,” \textit{Manuscript}, 2025.
\end{enumerate}
}

\vspace{3mm}
\noindent{Peer reviewed conference papers}
{%\footnotesize
\begin{enumerate}[{[I]}]\addtocounter{enumi}{5}
  \item \textbf{Z. Ni}, C. Zhang, M. Karlsson, and S. Gong, “Leveraging Deep Learning and Digital Twins to Improve Energy Performance of Buildings,” in \textit{2023 IEEE 3rd International Conference on Industrial Electronics for Sustainable Energy Systems (IESES)}, 2023.
  \item \textbf{Z. Ni}, C. Zhang, M. Karlsson, and S. Gong, “Edge-based Parametric Digital Twins for Intelligent Building Indoor Climate Modeling,” in \textit{2024 IEEE 20th International Conference on Factory Communication Systems (WFCS)}, 2024.
\end{enumerate}
}

\newpage 
% \vspace{5mm}

\noindent\textbf{Papers not included in this thesis:}

\vspace{3mm}

\noindent{Peer reviewed journal papers}
{%\footnotesize
\begin{enumerate}[{[I]}]\addtocounter{enumi}{7}
  \item Y. Liu, \textbf{Z. Ni}, M. Karlsson, and S. Gong, “Methodology for Digital Transformation with Internet of Things and Cloud Computing: A Practical Guideline for Innovation in Small-and Medium-Sized Enterprises,” \textit{Sensors}, vol. 21, no. 16, 2021.
  \item Y. Liu, S. Mousavi, Z. Pang, \textbf{Z. Ni}, M. Karlsson, and S. Gong, “Plant Factory: A New Playground of Industrial Communication and Computing,” \textit{Sensors}, vol. 22, no. 1, 2022.
  \item C. Zhang, \textbf{Z. Ni}, and C. Berger, “Spatial-Temporal-Spectral LSTM: A Transferable Model for Pedestrian Trajectory Prediction,” \textit{IEEE Transactions on Intelligent Vehicles}, vol. 9, no. 1, pp. 2836--2849, 2024.
  \item C. Zhang, J. Sprenger, \textbf{Z. Ni}, and C. Berger, “Predicting Pedestrian Crossing Behavior in Germany and Japan: Insights into Model Transferability,” accepted in \textit{IEEE Transactions on Intelligent Vehicles}, 2024.
\end{enumerate}
}

\vspace{3mm}
\noindent{Peer reviewed conference papers}
{%\footnotesize
\begin{enumerate}[{[I]}]\addtocounter{enumi}{11}
  \item \textbf{Z. Ni}, P. Eriksson, Y. Liu, M. Karlsson, and S. Gong, “Improving Energy Efficiency while Preserving Historic Buildings with Digital Twins and Artificial Intelligence,” in \textit{SBE21 Sustainable Built Heritage}, 2021.
  \item \textbf{Z. Ni}, Y. Liu, M. Karlsson, and S. Gong, “Link Historic Buildings to Cloud with Internet of Things and Digital Twins,” in \textit{The 4th International Conference on Energy Efficiency in Historic Buildings}, 2022.
  \item C. Zhang, AH. Kalantari, Y. Yang, \textbf{Z. Ni}, G. Markkula, N. Merat, and C. Berger, “Cross or Wait? Predicting Pedestrian Interaction Outcomes at Unsignalized Crossings,” in \textit{2023 IEEE Intelligent Vehicles Symposium}, 2023.
  \item C. Zhang, J. Sprenger, \textbf{Z. Ni}, and C. Berger, “Predicting and Analyzing Pedestrian Crossing Behavior at Unsignalized Crossings,” in \textit{2024 IEEE Intelligent Vehicles Symposium}, 2024.
\end{enumerate}
}

==> pdftopdfa <==
#! /usr/bin/env bash
filenames=${@%.pdf}
#### Use sRGB for now, proper color profile handling likely first in latex-3
#  -sColorConversionStrategy=UseDeviceIndependentColor 
for filename in ${filenames[@]}; do
  echo Converting ${filename}.pdf
  gs -dPDFA -dBATCH -dNOPAUSE              \
    -sColorConversionStrategy=RGB          \
    -sDEVICE=pdfwrite                      \
    -dPDFACompatibilityPolicy=3            \
    -sOutputFile=${filename}_pdfa_rgb.pdf  \
     ${filename}.pdf
  gs -dPDFA -dBATCH -dNOPAUSE              \
    -sColorConversionStrategy=CMYK         \
    -sDEVICE=pdfwrite                      \
    -dPDFACompatibilityPolicy=3            \
    -sOutputFile=${filename}_pdfa_cmyk.pdf \
     ${filename}.pdf
done


==> sammanfattning.tex <==
%%% sammanfattning.tex --- 
%% 
%% Filename: sammanfattning.tex
%% Description: 
%% Author: Ola Leifler
%% Maintainer: 
%% Created: Thu Oct 14 13:34:11 2010 (CEST)
%% Version: $Id$
%% Version: 
%% Last-Updated: Thu Apr 13 11:36:41 2017 (+0200)
%%           By: Ola Leifler
%%     Update #: 8
%% URL: 
%% Keywords: 
%% Compatibility: 
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Commentary: 
%% 
%%  Populärvetenskaplig sammanfattning av arbetet på svenska
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Change log:
%% 
%% 
%% RCS $Log$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Code:
% ✅✅

Utvecklingen av datadrivna digitala lösningar ger helt nya möjligheter i fastighetssektorn att förenkla driften. Med smart övervakning, prediktiv modellering och artificiell intelligens så går det att fatta bättre beslut och arbeta mer proaktivt. Kulturhistoriska byggnader är ett särskilt utmanande område där prediktivt underhåll är helt avgörande för att säkerställa ett långsiktigt bevarande för framtida generationer. Denna avhandling presenterar flera vetenskapliga framsteg för en datadriven drift av historiska byggnader där sakernas internet (Internet of Things, IoT), molnteknik, edge computing, digitala tvillingar och maskininlärning spelar en central roll. Dessa teknologier tillsammans möjliggör en helhetslösning som underlättar drift och underhåll för byggnadens bevarande utan att kompromissa med inomhusklimat och energieffektivitet.

Med målet att underlätta långsiktig övervakning av inomhusmiljö, presenteras i Artikel I en skalbar digitaliseringslösning som kombinerar ett IoT-baserat sensorsystem med edge- och molnteknik. Resultat visar att systemet har hög tillförlitlighet och att dess kombinationen av realtidsanalys och historiska data ger ett robustare underlag för beslut. I Artiklarna II och III vidareutvecklas konceptet med digitala tvillingar genom att även integrera ontologi-baserade datamodeller. Det ger tillsammans en mer enhetlig och komplett beskrivning av byggnadens, tekniska system och inomhusmiljö. Fallstudier vid Norrköpings Stadsteater och Löfstad slott i Östergötland visar att digitala tvillingar underlättar identifieringen av klimatrelaterade risker och därmed ger vägledning i bevarandearbetet.

Utifrån insamlade data undersöker Artiklar IV och VI hur djupinlärning kan användas för att förutsäga energianvändning i olika byggnader. Artikel IV utvärderar moderna djupinlärningsmodeller för både punktprognoser och sannolikhetsbaserade prognoser. Resultat visar att om predikterbara framtida externa faktorer inkluderas så förbättras prognosernas noggrannhet avsevärt. Studien belyser också hur olika driftförhållanden påverkar modellernas prestanda. Artikel VI kombinerar djupinlärning med digitala tvillingar för att identifiera möjligheter att minska energiförbrukningen och optimera driften.

Artiklar V och VII fokuserar på prediktiv modellering av inomhusklimat i olika byggnader. Artikel VII presenterar en edge-centrerad lösning som ett alternativ till molncentrerat system, vilket möjliggör snabb respons och skydd av integritetskänsliga data. Artikel V undersöker federerad djupinlärning, en metod där flera byggnader kan tränas med gemensamma klimatprognosmodeller utan att behöva dela rådata. Jämförelser mellan olika federerade inlärningsalgoritmer visar att dessa modeller kan ge snarlik hög prognosnoggrannhet som centraliserad inlärning, samtidigt som datasekretessen bibehålls. Resultaten ger viktiga insikter i hur man kan hantera spridda och heterogena miljödata för att stödja hållbar byggnadsförvaltning.

Genom att kombinera smart övervakning, digitala tvillingar och artificiell intelligens bidrar denna avhandling till att utveckla datadriven bevaring av historiska byggnader. De föreslagna metoderna underlättar drift, förebyggande underhåll och banar väg för en strategi för användning av digital teknologi inom kulturarvsbevarande.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% sammanfattning.tex ends here


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "demothesis"
%%% End: 

